Structural Biases for Improving Transformers on Translation into Morphologically Rich Languages

Machine translation has seen rapid progress with the advent of Transformer-based models. These models have no explicit linguistic structure built into them, yet they may still implicitly learn structured relationships by attending to relevant tokens. We hypothesize that this structural learning could be made more robust by explicitly endowing Transformers with a structural bias, and we investigate two methods for building in such a bias. One method, the TP-Transformer, augments the traditional Transformer architecture to include an additional component to represent structure. The second method imbues structure at the data level by segmenting the data with morphological tokenization. We test these methods on translating from English into morphologically rich languages, Turkish and Inuktitut, and consider both automatic metrics and human evaluations. We find that each of these two approaches allows the network to achieve better performance, but this improvement is dependent on the size of the dataset. In sum, structural encoding methods make Transformers more sample-efficient, enabling them to perform better from smaller amounts of data.

==> ethics_statement.tex <==
\section{Ethics Statement}

To our knowledge, the work presented here does not have directly applicable malicious use-cases. Translation is generally viewed as a beneficial resource for society to break down barriers between communities and aid in understanding.

\textbf{Intended use}
The intended use of this research is to improve machine translation systems. In particular, we examined the ways that our proposed methods can help deal with more complex sentences in morphologically rich languages, as well as improvements for smaller datasets and low-resource languages.

\textbf{Failure modes}
Mistranslation can be a serious issue, and we do not see this tool replacing professional translators, especially as the stakes of the translation increase, such as geopolitical situations.

\textbf{Biases}
As with all large-scale machine learning models, the models presented here likely capture the biases in the datasets which reflect the biases of society \cite{parrots}. In particular, the Turkish Open Subtitles dataset contains many crude and problematic pairs from programs intended for mature audiences.

\textbf{Misuse potential}
Improved translation systems provide an opportunity for malicious actors to spread misinformation more easily by translating fake news into many languages

\textbf{Potential harm to vulnerable populations}
The techniques we proposed in this paper have the largest effect on smaller datasets. In practice, most widely spoken languages have a plethora of data thanks to the internet. Languages that use small datasets in practice are low-resource languages, and those tend to come from marginalized communities.

==> page_breaks.tex <==
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$
$\newpage$

